Fully-Trainable Deep Matching

Deep Matching (DM) is a popular high-quality method for quasi-dense image matching. Despite its name, however, the original DM formulation does not yield a deep neural network that can be trained end-to-end via backpropagation. In this paper, we remove this limitation by rewriting the complete DM algorithm as a convolutional neural network. This results in a novel deep architecture for image matching that involves a number of new layer types and that, similar to recent networks for image segmentation, has a U-topology. We demonstrate the utility of the approach by improving the performance of DM by learning it end-to-end on an image matching task.

==> experiments.tex <==
\section{Experiments}

\subsection{Evaluation of descriptor network architectures}

We base our descriptor networks on the initial layers of VGG-16, which has shown excellent
performance in visual recognition tasks. Specifically, we have a number of $3\times3$ convolutions with 64 output channels, followed by max pooling with a stride of 2, then a further set of $3\times3$ convolutions with 128 output channels. We experiment with varying the number of convolution layers before and after the max pool, which has the effect of changing both the receptive field of the network and the number of parameters. 

Since the Deep Matching architecture operates on patches of size $4\times4$, we have a final $4\times4$ convolution with 128 output channels, which at evaluation time is applied
with stride 4 to the first image and with stride 1 to the second image.


\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
        Name  & RF Size      & Number of Parameters \\
        Net22 & $20\times20$ & todo \\
        Net23 & $24\times24$ &     \\            
        Net32 & $22\times22$ &\\
        Net33 & $26\times26$ &\\
        Net44 & $32\times32$ &\\
    \end{tabular}
    \caption{Descriptor network architectures. The name Net$xy$ denotes $x$ $3\times3$ convolutions prior to the max pool and $y$ after it.}
    \label{tab:descnets}
\end{table}

\subsection{Training procedure}
% SPP-style training
% hard negative mining etc

\subsection{Combining input scales}

\subsection{Results on Sintel}
%table: test results

%table: validation sequences

%talk a bit about difficult frames, smoke effects etc.


==> scratch.tex <==
\appendix
\section{Calculations}



In this section we discuss some implementation details concerning how score maps are discretized in the implementation. We denote with a bar the discretized signals, and, for $l = 0, 1, 2, \dots L$, define them as follows:
\begin{align*}
\bar S_{l}(\bk_l|\bi_l) &=
S_{l}(\bq|\bp),
&
\bar S_{l+\frac{1}{2}}(\bk_{l+1}|\bi_l) &=
S_{l+\frac{1}{2}}(\bq|\bp),\\
\bar Q_{l}(\bk_l|\bi_l) &=
Q_{l}(\bq|\bp),
&
\bar Q_{l+\frac{1}{2}}(\bk_{l+1}|\bi_l) &=
Q_{l+\frac{1}{2}}(\bq|\bp),
\end{align*}
where coordinates $\bp$ and $\bq$ are sampled as
\begin{align*}
\&
\end{align*}
and $\tau_l$ is the adjustment:


The coordiante $\bq$ in the target image is sampled relative to $\bp$ within a range of $R_0$ samples. The sampling stride $\gamma_0$ of $\bq$ does not need to be the same as the sampling stride $\alpha_0$ of $\bp$; in the following, we assume for simplicity that $\gamma_0|\alpha_0$. Note that the sampling stride of $\bq$ is halved with each successive level; this is to reduce redundancy in the representation of smooth coarse score maps.

Next, we show how these choices result in simple implementations of the max pooling and aggregation layers as CNN building blocks.

\paragraph{Max pooling.} Recall that $S_{l+1/2}(\bq|\bp)$ is obtained by pooling $S_{l}(\bq'|\bp)$ in the window $\|\bq' - \bq\|_\infty \leq 2^l \eta_0$. We now show that the discretized version $\bar S_{l+1/2}(\bk_{l+1}|\bi_l)$ is obtained from $\bar S_{l}(\bk_{l}|\bi_l)$ by applying the standard CNN max pooling operator with certain parameters. In order to do so, replace $\bq$ an $\bq'$ with their expressions in $\bk_{l+1}$ and $\bk_l$. For the pooling window, this results in the condition:
\[
\left[
R_l - 2R_{l+1} -\frac{\eta_0}{\gamma_0}
\right]
+ 2(\bk_{l+1}-1) 
\leq
\bk_{l} - 1 
\leq
\left[R_l - 2R_{l+1}  + \frac{\eta_0}{\gamma_0}\right]
+ 2(\bk_{l+1}-1)
\]
where all terms are integer since $\gamma_0 | \eta_0$ by assumption. This corresponds to pooling in a window of
\[
W = 1 +  2\frac{\eta_0}{\gamma_0}
\]
samples and with $2$ as stride. Furthermore, recall that the range of variable $\bk_{l+1}$ is $1 \leq \bk_{l+1} \leq 2R_{l+1}$. Thus the first and last pooled samples in $\bk_l$ are obtained by setting $\bk_{l+1}$ to either 1 or $2R_{l+1}$ in the equation above, which results in:
\begin{align*}
   \bk_{l}^{\text{first}}&= 1 - P_-
   &
   \text{thus\ } P_- &= \frac{\eta_0}{\gamma_0} + (2R_{l+1} - R_l),
   \\
   \bk_{l}^{\text{last}}&= 2R_l + P_+
   &
   \text{thus\ }  P_+ &= P_- - 1.
\end{align*}
Here $P_-$ and $P_+$ are respectively the left and right padding applied by the max pooling operator.

Finally, note that the range $R_{l+1}$ of the pooled signal can be made arbitrary large as this simply results in more padding. However, the informative part of the signal is obtained when $2R_{l+1} \approx R_l$, so we set:
\[
 R_{l+1} = \left\lceil \frac{R_l}{2} \right\rceil.
\]
With this choice, the  padding $P_-$ is equal to half of the pooling window size (plus one if $R_l$ is not an even number).

\paragraph{Aggregation.} For aggregation, recall that 
$S_{l+1}(\bq|\bp)$ is obtained by summing four samples $S_{l+\frac{1}{2}}(\bq + 2^l\bdelta_i| \bp + 2^l\bdelta_i)$. We now show that this reduces to summing four slices of the type $\bar S_{l+1}(\cdot | \bi_{l+1})$.

To do so, note that substituting in $\bq + 2^l\bdelta_i$ the expression of $\bq$ in $\bk_{l+1}$ results in
\[
\bq + 2^l\bdelta_i
=
2^{l+1}\gamma_0 (\bk_{l+1} - 1 - R_{l+1}) + (\bp + 2^l\bdelta_i).
\]
Thus, the fact that in the coordiante $\bq$ is sampled relatively to $\bp$ means that the shift applied to $\bq$ is absorbed in the shift applied to $\bp$; this means that $\bar S_{l+1}(\cdot | \bi_{l+1})$ is obtained by directly averaging four slices $\bar S_{l+1/2}(\cdot | \bi_l)$ for appropriate values of the index $\bi_l$. Next, we identifying the indices of such slices. Substituting in $\bp + 2^l\bdelta_i$ the expression of $\bp$ in $\bi_{l+1}$ results in:
\begin{align*}
\bp + 2^l\bdelta_i
&=
\alpha_0 
(\bi_{l+1} - 1 + \tau_{l+1}) + \beta_0
+ 2^{l-1}\delta_0 \bepsilon_i \\
&=
\alpha_0 
\left(
\underbrace{
\bi_{l+1} + \tau_{l+1} - \tau_l + 2^l \frac{\delta_0}{2\alpha_0} \bepsilon_i}_{\bi_l} 
- 1 + \tau_l
\right) 
+ \beta_0.
\end{align*}
We distinguish two cases. If $l \geq 1$, $\tau_l = \tau_{l+1}$ so that $\tau_{l+1}-\tau_l=0$. Furthermore, since $\alpha_0 | \delta_0$, the coefficient of the integer vector $\bepsilon_i$ is integer. Thus, $\bar S_{l+1}(\cdot | \bi_{l+1})$ is obtained by averaging the slices $\bar S_{l+1/2}(\cdot | \bi_l)$ given by
\[
 \bi_l = \bi_{l+1} + 2^l \frac{\delta_0}{2\alpha_0} \bepsilon_i,\qquad i=1,2,3,4.
\]
However, at the first level $l=0$, due to the division by $2$, the coefficient multiplying $\bepsilon_i$ is in general not an integer number. For $l=0$ we also have $\tau_0=0$ and one obtains the special case:
\begin{align*}
 \bi_0 
 = \bi_{1} - \tau_0 + \frac{\delta_0}{2\alpha_0} \bepsilon_i
 =
 \bi_{1}
+ \left\lceil \frac{\delta_0}{2\alpha_{0}} \right\rceil
+ \frac{\delta_0}{\alpha_0} 
\frac{\bepsilon_i- 1}{2},
\quad
i=1,2,3,4.
\end{align*}
Note that $\bepsilon_i - 1$ contains even numbers ($0$ and $-2$), so the expression above is integer. This explains the need for the shift $\tau_l$ in the sampling of $\bp$.

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Accuracy@T & DM with default param & DM with learned param & improvements \\ \hline
acc@10     & 85.40\%                    & 85.40\%                    & 0.00\%       \\ \hline
acc@9      & 84.86\%                    & 84.88\%                    & 0.02\%       \\ \hline
acc@8      & 84.18\%                    & 84.22\%                    & 0.04\%       \\ \hline
acc@7      & 83.29\%                    & 83.36\%                    & 0.07\%       \\ \hline
acc@6      & 82.08\%                    & 82.16\%                    & 0.08\%       \\ \hline
acc@5      & 80.31\%                    & 80.40\%                    & 0.09\%       \\ \hline
acc@4      & 77.42\%                    & 77.51\%                    & 0.09\%       \\ \hline
acc@3      & 72.11\%                    & 72.15\%                    & 0.04\%       \\ \hline
acc@2      & 60.57\%                    & 60.46\%                    & -0.11\%      \\ \hline
acc@1      & 30.53\%                    & 30.36\%                    & -0.17\%      \\ \hline
\end{tabular}
\end{center}
\caption{Matching performance comparison on KITTI 2012 training set. Accuracy@$T$ measures the proportion of "correct" pixels from the first image with respect to the total number of pixels, $T$ is the pixel threshold allowing displacement. We learn our DM parameters based on Flying chair dataset. Apart from the learned parameters, both DM results are based on DM with $\infty$ neighbor and $1/2$ downscale. }
\label{table:matchingres}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Accuracy@T & DM with default param & DM with learned param & improvements \\ \hline
acc@10     & 85.11\%               & 85.02\%               & -0.09\%      \\ \hline
acc@9      & 84.61\%               & 84.54\%               & -0.07\%      \\ \hline
acc@8      & 84.01\%               & 83.97\%               & -0.04\%      \\ \hline
acc@7      & 83.29\%               & 83.28\%               & -0.01\%      \\ \hline
acc@6      & 82.26\%               & 82.28\%               & 0.02\%       \\ \hline
acc@5      & 81.03\%               & 81.09\%               & 0.06\%       \\ \hline
acc@4      & 79.17\%               & 79.26\%               & 0.09\%       \\ \hline
acc@3      & 76.37\%               & 76.46\%               & 0.09\%       \\ \hline
acc@2      & 69.69\%               & 69.82\%               & 0.13\%       \\ \hline
acc@1      & 48.40\%               & 48.51\%               & 0.11\%       \\ \hline
\end{tabular}
\end{center}
\caption{Matching performance comparison on SINTEL final training set. Accuracy@$T$ measures the proportion of "correct" pixels from the first image with respect to the total number of pixels, $T$ is the pixel threshold allowing displacement. We learn our DM parameters based on Flying chair dataset. Apart from the learned parameters, both DM results are based on DM with $\infty$ neighbor and $1/2$ downscale. }
\label{table:matchingres}
\end{table}

\begin{table}[h!]
\begin{tabular}{|l|l|l|l|}
\hline
method                     & Acc@10 KITTI12                 & Acc@10 Sintel final    & Acc@10 Mikolajczyk            \\ \hline
SIFT-NN                    & 48.9\%                         & 68.4\%                 & 67.4\%                       \\ \hline
HOG-NN                     & 53.7\%                         & 71.2\%                 & n/a                          \\ \hline
KPM                        & 53.6\%                         & 73.8\%                 & n/a                          \\ \hline
GPM                        & 66.1\%                         & 81.2\%                 & 30.3\%                       \\ \hline
SIFT-flow                  & 67.3\%                         & 89.0\%                 & n/a                          \\ \hline
SLC                        & 74.8\%                         & 82.4\%                 & n/a                          \\ \hline
DaisyFF                    & 79.6\%                         & 87.3\%                 & 41.0\%                       \\ \hline
NRDC                       & n/a                            & n/a                    & 69.2\%                       \\ \hline
DM |1/2| $\infty$          & 85.6\%                         & 89.2\%                 & 65.7\%                       \\ \hline
DM |1/4| $\infty$          & 80.0\%                         & 83.5\%                 & 87.8\%                       \\ \hline
Ours |1/4| $128$           & 84.3\%                         &                        &                              \\ \hline
Ours+learning              &                                &                        &                              \\ \hline
\end{tabular}
\caption{Matching performance comparison based on accuracy@10. Accuracy@10 measures the proportion of "correct" pixels from the first image with respect to the total number of pixels. DM |1/2| $\infty$ indicates that DM with downscale 1 and $\infty$ means for no restriction on neighbourhood. All results from DM are produced by the DM original code. Notice Our implementation for DM is comparable to the original one, and ours can significant improve the performance by optimizing the parameters through back-propagation algorithm.}
\label{table:matchingres}
\end{table}


\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Train set     & Model variants                     & Sparse EPE R80 & Accuracy@10 R128 \\ \hline
None          & DM baseline                        & 3.819          & 0.9291           \\ \hline
Sintel Mini   & Exponents                          & 3.694          & 0.9311           \\ \hline
Sintel Mini   & Exponents \& Score weights         & 3.607          & 0.9298           \\ \hline
Sintel Mini   & Exponents \& wb                    & 3.6254         & 0.9307           \\ \hline
Flying Chairs & Exponents                          & 3.7457         & 0.931            \\ \hline
\end{tabular}
\caption{Ablation studies show that the performance of our model is improved after training}
\label{label:ablation}
\end{center}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Base network  & Parameters Learned & Sparse EPE R80 & Accuracy@10 R128 \\ \hline
None          & None               & 3.819          & 0.9291           \\ \hline
VGG16         & None               & 3.4128         & 0.932            \\ \hline
\end{tabular}
\caption{HOG vs VGG shallow network.}
\label{label:features}
\end{center}
\end{table}


